Data-driven Upsampling of Point Clouds

High quality upsampling of sparse 3D point clouds is critically useful for a wide range of geometric operations such as reconstruction, rendering, meshing, and analysis. In this paper, we propose a data-driven algorithm that enables an upsampling of 3D point clouds without the need for hard-coded rules. Our approach uses a deep network with Chamfer distance as the loss function, capable of learning the latent features in point clouds belonging to different object categories. We evaluate our algorithm across different amplification factors, with upsampling learned and performed on objects belonging to the same category as well as different categories. We also explore the desirable characteristics of input point clouds as a function of the distribution of the point samples. Finally, we demonstrate the performance of our algorithm in single-category training versus multi-category training scenarios. The final proposed model is compared against a baseline, optimization-based upsampling method. Results indicate that our algorithm is capable of generating more uniform and accurate upsamplings.

==> later_half_revised_version.tex <==
\section{Results and Discussions}
\subsection{Inner-class evaluation}\label{inner eval}
As is stated in section\ref{Experiment Details}, we conduct parametric studies with twelve different cases to evaluate the upsampling capability of our algorithm. The resulting average test Chamfer losses for each category are shown in table \ref{tab: inner}. The best performances with equal scaling factor of each category has been marked in bold. We report the accuracy and coverage values as well in Appendix, which show a close trendency to table \ref{tab: inner}.
Among all the best cases, the biggest test Chamfer loss is less than $1.7\times10^{-3}$(minimum $0.285\times10^{-3}$). When scaling factor is doubled, the most significant increase in Chamfer loss is only around 8\%. Referring to the visualizations of reconstruction quality with various Chamfer loss values, we can deem that overall our upsampling algorithm is excellent and stable in addressing upsampling tasks of different objects with multiple scaling factors. 

An interesting fact is that uniform sampling outperforms curvature-based sampling in all the cases where scaling factor is 4 or 8. But in 4 of 7 categories, points near the object outlines result in finer reconstruction quality. Since Qi at el.\cite{6} have mentioned that the critical points contributing more to the features usually lie around the edges and outlines of the object, we originally expected points downsampled based on curvature values would be more efficient in reconstruction. Because points near the object skeletons normally have larger curvatures. A possible reason is that the input points concentrate too much on the edges so that the resulting point cloud is pretty ununiform. This ununiformity may decrease the error distance from prediction to ground truth since features like sharp edges or curve surfaces need more points to describe. Meanwhile, it inevitably gives rise to the error distance from ground truth to prediction. Because the total number of points is fixed, there must be less points on the flat surfaces. In cases where the scaling factor is small, the side effect of this ununiformity is not distinctly revealed since the total number of points is still adequate to cover the flat areas. As SF becomes larger, the unbalanced point distribution eventually results in a dominant threat to the upsampling performance. To verify our hypothesis explained above, a conbined sampling method with various combining ratios is introduced in section \ref{further}. However, as the results demonstrate, normal information doesn't help to improve the upsampling quality in all the cases. 

\begin{table*}[!htb]
\centering
\renewcommand{\arraystretch}{2}
\begin{tabular}{ |c||c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{3}{*}{} SF & \multicolumn{4}{c|}{2} & \multicolumn{4}{c|}{4} & \multicolumn{4}{c|}{8}\\ 
\cline{1-13}
                    Sample & \multicolumn{2}{c|}{Uniform} & \multicolumn{2}{c|}{CB} & \multicolumn{2}{c|}{Uniform} & \multicolumn{2}{c|}{CB} & \multicolumn{2}{c|}{Uniform} & \multicolumn{2}{c|}{CB}\\
\cline{1-13}
                    Normal & w/o & w/ & w/o & w/ & w/o & w/ & w/o & w/ & w/o & w/ & w/o & w/\\
\hline
Category & \multicolumn{12}{c|}{Test Chamfer Loss($\times10^{-3}$)}\\
\hline
Airplane & \textbf{0.285} & 0.301 & 0.289 & 0.311 & \textbf{0.294} & 0.316 & 0.313 & 0.343 & \textbf{0.319} & 0.340 & 0.356 & 0.402\\ 
 \hline
Bench & 0.814 &	1.154 &	\textbf{0.771} &	2.480 &	\textbf{0.822} &	1.089 &	0.940 &	1.297 &	\textbf{0.865} &	1.273 &	0.996 &	1.391\\ 
 \hline
Boat & 0.923 &	1.325 &	\textbf{0.899} &	1.410 &	\textbf{0.971} &	1.359 &	1.008 &	1.449 &	\textbf{1.000} &	1.420 &	1.043 &	1.206\\ 
 \hline
Car & \textbf{0.720} &	0.751 &	0.721 &	0.738 &	\textbf{0.729} &	0.763 &	0.767 &	0.806 &	\textbf{0.755} &	0.794 &	0.816 &	0.866\\ 
 \hline
Chair & \textbf{1.322} &	1.387 &	1.335 &	1.367 &	\textbf{1.353} &	1.388 &	1.792 &	1.868 &	\textbf{1.414} &	1.462 &	1.933 &	2.040\\ 
 \hline
Lamp & 1.530 &	2.039 &	\textbf{1.528} &	2.161 &	\textbf{1.571} &	2.028 &	1.657 &	2.163 &	\textbf{1.635} &	2.254 &	1.824 &	2.665\\ 
 \hline
Table & 1.185 &	1.196 &	\textbf{1.181} &	1.196 &	\textbf{1.194} &	1.219 &	1.389 &	1.418 &	\textbf{1.231} &	1.258 &	1.549 &	1.593\\ 
 \hline
\end{tabular}
\caption{\label{tab: inner} Evaluation of networks trained on 7 categories respectively under twelve conditions. The lowest test Chamfer loss for each scaling factor is marked in bold.}
\end{table*}


\begin{table*}[!htb]
\centering
\renewcommand{\arraystretch}{2}
\begin{tabular}{ |c||c|c|c|c|c|c|c|}
\hline
Training Category & Airplane & Bench & Boat & Car & Chair & Lamp & Table\\ 
\hline
Evaluation Category & \multicolumn{7}{c|}{Test Chamfer Loss($\times10^{-3}$)}\\
\hline
Airplane & \textbackslash & 24.321 & 102.293 & 23.312 & 9.943 & 3.530 & 11.599\\ 
 \hline
Bench & 77.826 & \textbackslash & 35.462 & 44.513 & 1.519 &	6.089 &	1.649\\ 
 \hline
Boat & 3.953 & 11.938 &	\textbackslash &	4.273 &	4.933 &	2.067 &	10.881\\ 
 \hline
Car & 5.152 & 5.406 & 1.543 & \textbackslash & 2.601 & 3.163 &	4.418\\ 
 \hline
Chair & 30.484 & 5.982 & 20.687 & 17.633 & \textbackslash & 11.387 & 4.754\\ 
 \hline
Lamp & 12.609 &	35.19 &	18.575 & 56.709 & 8.846 & \textbackslash & 12.545\\ 
 \hline
Table & 72.059 & 5.909 & 67.493 & 47.852 & 4.883 & 17.199 & \textbackslash\\ 
 \hline
\end{tabular}
\caption{\label{tab: inter} Inter-class evaluating of the networks trained by each category. Uniformly distributed points are used during training as input point clouds. $SF=8$.}
\end{table*}

\begin{table*}[!htb]
\centering
\renewcommand{\arraystretch}{2}
\begin{tabular}{ |c||c|c|c|c|c|c|c|}
\hline
Evaluation Category & Airplane & Bench & Boat & Car & Chair & Lamp & Table\\ 
\hline
Test Chamfer Loss($\times10^{-3}$) & 0.529 & 0.825 & 0.892 & 0.854 & 1.807 & 1.888 & 1.644\\ 
 \hline
\end{tabular}
\caption{\label{tab: multi} Evaluation of the network trained on mutiple categories. The upsampling condition is the same as table. \label{tab: inter}.}
\end{table*}

\subsection{Inter-class and multi-class evaluation}
Based on the results from table \ref{tab: inner}, we want to extensively explore the generality of our models trained on each single category or multiple categories. As a case study, all the networks are trained under such conditions: $SF=8$, uniformly downsampled point clouds and without normal information. Because when $SF=8$, least input information is given and results in the most significant variances in test Chamfer loss among all the categories. Then we choose the other two conditions which provide the best performance according to table \ref{tab: inner}. All the networks trained in the previous experiment category has been preserved. They are directly tested on the other 6 categories. The outcome Chamfer losses are displayed in table \ref{tab: inter}. We can observe an evident increase in average loss because of the lack of learned experience for other categories. Still, the network trained by chairs achieves $4.877\times10^{-3}$ on average test loss. This might come from the abundant variance in chair models. Bench models are relatively consistent in style and structure with only 5 children types. While chair models, apart from some similar designs, in total include 23 various children types such as arm chairs, folding chairs, recliners or even wheel chairs. Therefore, the network which is trained on chairs and tested on benches, provides less increase percentage in test performance than the network which is trained on benches and tested on chairs. Thus, we can conclude that higher variance in training sets can improve the overall generality of final network model.

However, higher variance in training sets usually requires more complex network architecture or leads to worse performance. To inspect our algorithm on addressing this issue, another network model is trained based on a balanced training set generated from each category. Referring to table \ref{tab: multi}, comparing with corresponding results in table \ref{tab: inner}, test losses of benches and boats even decrease. At the expense that the average test loss rises solely from 1.031 to 1.205, this model is able to upsample point clouds of all 7 categories with relatively high quality and precision. More visual results can be found in appendix XXX.

\subsection{Further discussions}\label{further}
According to the hypothesis we propose in section \ref{inner eval}, a mixture sampling method is designed to provide a potential superior input point distribution for upsampling. We introduce a new parameter, combining ratio $\alpha\in[0,1]$, to represent the percentage of points downsampled by curvature-based strategy. The other part of points are downsampled uniformly without repetition. As a parametric study, we create 11 groups of input point clouds from airplane category with $SF=8$ and an increment of $0.1$ in $\alpha$ each time. The test cases are identical to those we use in table \ref{tab: inner}. Figure XXX summarizes the relationship between $\alpha$ and the corresponding test Chamfer loss. As shown, $\alpha=0.1$ or $\alpha=0.2$ both provide higher upsampling quality over the uniformly sampled points($\alpha=0$). The results exhibit the significance of critical points around the outlines on generalizing the whole shape of the object. Within a certain range of mixture(less than about $20\%$ in this case), those critical points help to decrease the Chamfer loss in that the local features around edges and corners are better represented. But the input point is also becoming less uniform as $\alpha$ get larger. Eventually, the improvement resulted from edge points cannot make up for the lack of points on the flat surfaces. The accuracy and coverage values reported in Appendix. further verifies our presumption. Also, we can observe a gradual growth of test Chamfer loss after a inflection point($20\%$) in the curve shown in figure XXX.

As a comparison with the model we obtained from the best combining ratio, we utilize EAR\cite{XXX}, a state-of-the-art method for optimization-based point cloud upsampling method, to complete the same task. Figure XXX illustrates that our algorithm provides more precise upsampling results over EAR method.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Conclusions}
This work presents a deep learning algorithm aiming at enriching the number of points in a sparse point cloud with flexible scaling factors. Through upsampling, our goal is to sense and supplement the point cloud with more information learned on other existing point clouds with similar global features. Instead of using any human defined priors, we take advantage of the outstanding ability of deep networks to obtain latent features for a certain object category. Then these latent features assist the point cloud upsampling
with correct category judgment so that some common global features learned from the same category can be naturally exploited.

We successively explore the effect of two different distributions for input point cloud sampling. Based on the experiment outcomes, a further parametric study on the combining ratio for points produced by these two sampling strategies is conducted to identify the benefit and side effect of using critical points for upsampling. As SF rises, points lying on the outlines of an object is capable of forming finer description of the critical features around the edges. Meanwhile, the descent of point density in areas far from edges causes the scarcity of points in these areas during the upsampling, which unavoidably decrease the accuracy in current evaluation metric. However, in real application, the ultimate goal is usually to reconstruct a precise surface based on a dense point cloud. Less points in flat areas won't be a very severe problem since almost all the surface reconstruction methods assume smooth and flat surfaces between the given points. In this manner, our immediate next move is to define more practical metrics to evaluate the resulting dense point cloud so that we can expand the applications of our algorithm.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Future Work}
Our current model is trained on point clouds sampled from ShapeNetCore. As we inspect the meshes utilized in our training, we find out that part of the meshes have flaws like open meshes or double-sided surfaces. These flaws lead to some incorrect normal calculation, which is a potential reason why normal information doesn't enhance the upsampling quality. An alternative way is to obtain the normal vectors only depending on the vertex coordinates. We believe it will bypass the defect in mesh surfaces and provide more accurate normal vectors so that we can extensively verify its influence.  

Another limitation of this study is that our deep network is proficient at reconstructing the global features that are frequently occurred in the category. For those features that rarely exist or never occur in the training sets, the upsampling quality is not as good as the former ones. To address this problem, we can investigate the possibility of replenishing latent features learned from patch scale.



==> results_con_revision_Jiang.tex <==
\section{Results and Discussions}
\subsection{Inner-class evaluation}\label{inner eval}
As is stated in
% section?
\ref{Experiment Details}, we conduct parametric studies with 12 different cases to test(evaluate，?) the upsampling quality(ability?) of our algorithm when trained and tested on point clouds from the same category. The resulting average test Chamfer losses
% Chamfer loss or distance for the whole paper?
for each category are shown in table \ref{tab: inner}. The best case for each scaling factor in each category has been marked in bold. 
% The best case with equal scaling factor of each category 
Among all the best cases, the largest(biggest) test Chamfer loss value is less than $1.7\times10^{-3}$(minimum $0.285\times10^{-3}$). When scaling factor is doubled, the most significant increase in Chamfer loss is only around 8\%. Referring to the visualizations of reconstruction quality with various Chamfer loss values, we can deem that overall our upsampling algorithm is excellent and stable in addressing upsampling tasks of different models with multiple scaling factors. 
% should we give the reader a feeling of chamfer loss like nuc?

An interesting fact is that uniform sampling outperforms curvature-based sampling in all the cases where scaling factor is 4 or 8. But in 4 of 7 categories, curvature-based sampling method is better(?). Since Qi at el.\cite{6} have mentioned that the critical points usually lie around the edges(要不就用outline)
% critical point sets CS, those contributed to the max pooled feature, summarizes the skeleton of the shape.
 and outlines of the model, we originally expected curvature-based sampling will be overall better(more effective?) because points near edges normally have larger curvatures. A possible reason is that the curvature-based sampling concentrates too much on the points with larger curvatures so that the whole sampled point cloud is pretty ununiform. This ununiformity may decrease the error distance from prediction to ground truth since features like sharp edges or curve surfaces need more points to describe. Meanwhile, it will inevitably give rise to the error distance from ground truth to prediction. Because the total number of points is fixed, there must be less points on the flat surfaces. In cases where the scaling factor is small, the side effect of this ununiformity is not distinctly revealed(obvious?) due to that the total number of points is still adequate.（if all the points are on the edge?） As SF becomes larger, the unbalanced sampling eventually results in a dominant threat to the upsampling performance. To verify our hypothesis explained above, a conbined sampling method with various combining ratios is introduced in section \ref{further}. Unlike the effect of different sampling methods, normal information doesn't help to improve the upsampling quality in all the cases. 

\begin{table*}[!htb]
\centering
\renewcommand{\arraystretch}{2}
\begin{tabular}{ |c||c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{3}{*}{} SF & \multicolumn{4}{c|}{2} & \multicolumn{4}{c|}{4} & \multicolumn{4}{c|}{8}\\ 
\cline{1-13}
                    Sample & \multicolumn{2}{c|}{Uniform} & \multicolumn{2}{c|}{CB} & \multicolumn{2}{c|}{Uniform} & \multicolumn{2}{c|}{CB} & \multicolumn{2}{c|}{Uniform} & \multicolumn{2}{c|}{CB}\\
\cline{1-13}
                    Normal & w/o & w/ & w/o & w/ & w/o & w/ & w/o & w/ & w/o & w/ & w/o & w/\\
\hline
Category & \multicolumn{12}{c|}{Test Chamfer Loss($\times10^{-3}$)}\\
\hline
Airplane & \textbf{0.285} & 0.301 & 0.289 & 0.311 & \textbf{0.294} & 0.316 & 0.313 & 0.343 & \textbf{0.319} & 0.340 & 0.356 & 0.402\\ 
 \hline
Bench & 0.814 &	1.154 &	\textbf{0.771} &	2.480 &	\textbf{0.822} &	1.089 &	0.940 &	1.297 &	\textbf{0.865} &	1.273 &	0.996 &	1.391\\ 
 \hline
Boat & 0.923 &	1.325 &	\textbf{0.899} &	1.410 &	\textbf{0.971} &	1.359 &	1.008 &	1.449 &	\textbf{1.000} &	1.420 &	1.043 &	1.206\\ 
 \hline
Car & \textbf{0.720} &	0.751 &	0.721 &	0.738 &	\textbf{0.729} &	0.763 &	0.767 &	0.806 &	\textbf{0.755} &	0.794 &	0.816 &	0.866\\ 
 \hline
Chair & \textbf{1.322} &	1.387 &	1.335 &	1.367 &	\textbf{1.353} &	1.388 &	1.792 &	1.868 &	\textbf{1.414} &	1.462 &	1.933 &	2.040\\ 
 \hline
Lamp & 1.530 &	2.039 &	\textbf{1.528} &	2.161 &	\textbf{1.571} &	2.028 &	1.657 &	2.163 &	\textbf{1.635} &	2.254 &	1.824 &	2.665\\ 
 \hline
Table & 1.185 &	1.196 &	\textbf{1.181} &	1.196 &	\textbf{1.194} &	1.219 &	1.389 &	1.418 &	\textbf{1.231} &	1.258 &	1.549 &	1.593\\ 
 \hline
\end{tabular}
\caption{\label{tab: inner} Chamfer distance of evaluation of networks trained using 7 categories separately under 12 conditions. balabalabala}
\end{table*}



\begin{table*}[!htb]
\centering
\renewcommand{\arraystretch}{2}
\begin{tabular}{ |c||c|c|c|c|c|c|c|}
\hline
Training Category & Airplane & Bench & Boat & Car & Chair & Lamp & Table\\ 
\hline
Evaluation Category & \multicolumn{7}{c|}{Test Chamfer Loss($\times10^{-3}$)}\\
\hline
Airplane & \textbackslash & 24.321 & 102.293 & 23.312 & 9.943 & 3.530 & 11.599\\ 
 \hline
Bench & 77.826 & \textbackslash & 35.462 & 44.513 & 1.519 &	6.089 &	1.649\\ 
 \hline
Boat & 3.953 & 11.938 &	\textbackslash &	4.273 &	4.933 &	2.067 &	10.881\\ 
 \hline
Car & 5.152 & 5.406 & 1.543 & \textbackslash & 2.601 & 3.163 &	4.418\\ 
 \hline
Chair & 30.484 & 5.982 & 20.687 & 17.633 & \textbackslash & 11.387 & 4.754\\ 
 \hline
Lamp & 12.609 &	35.19 &	18.575 & 56.709 & 8.846 & \textbackslash & 12.545\\ 
 \hline
Table & 72.059 & 5.909 & 67.493 & 47.852 & 4.883 & 17.199 & \textbackslash\\ 
 \hline
\end{tabular}
\caption{\label{tab: inter} Chamfer distance of using testing point clouds from 7 categories to evaluate the networks trained on each category separately. balabalabala}
\end{table*}

\begin{table*}[!htb]
\centering
\renewcommand{\arraystretch}{2}
\begin{tabular}{ |c||c|c|c|c|c|c|c|}
\hline
Evaluation Category & Airplane & Bench & Boat & Car & Chair & Lamp & Table\\ 
\hline
Test Chamfer Loss($\times10^{-3}$) & 0.529 & 0.825 & 0.892 & 0.854 & 1.807 & 1.888 & 1.644\\ 
 \hline
\end{tabular}
\caption{\label{tab: multi} Chamfer distance of evaluation on each category by multi-class trained network. balabalabala}
\end{table*}

\subsection{Inter-class and multi-class evaluation}
Based on the results from table \ref{tab: inner}, we want to extensively explore the generality of our models trained on each single category or multiple categories. As a case study, all the models are trained under such conditions: $SF=8$, uniform sampling and without normal information. Because(We find that) when $SF=8$, least input information is given and results in the most significant variances in test Chamfer loss among all the categories.(?) Then we (decide the rest conditions by their performance) according to table \ref{tab: inner}. 7 models trained on each single(All the models trained in the previous experiment) category has been saved(preserved) in the previous experiment. They are continuously utilized(directly tested here on....) when evaluated on test cases from the other 6 categories. The resulting(outcome) Chamfer losses for each model are displayed in table \ref{tab: inter}. We can observe an evident increase in average loss because of the lack of learned experience for other categories. Still, the model trained from chair achieves $4.877\times10^{-3}$ on average test loss. This might come() from the abundant variance in chair models. A indirect proof can be found between chair and bench models.（？） Bench models are relatively consistent in style and structure with only 5 children types, while chair models, apart from some alike() designs, in total include(are divided into) 23 various children types such as arm chairs, folding chairs, recliners or even wheel chairs. Therefore, the model which is trained on chairs and tested on benches, provides less increase percentage in test performance than the model which is trained on benches and tested on chairs. We can conclude that higher variance in training sets can improve the overall generality of final network model. 
% model 和 CAD model总是掺杂一起说好吗？
% 找一些bench和chair的模型说明这个variance的问题

However, higher variance in training sets usually takes more complex training networks and leads to worse performance. To inspect our algorithm on addressing this issue, another network model is trained based on a balanced training set generated from each category and tested on the same test cases as the previous experiments.(说了好多次了) Referring to table \ref{tab: multi}, comparing with corresponding results in table \ref{tab: inner}, test losses of benchs and boats() even decrease. At the expense that the average test loss rises solely from 1.031 to 1.205, this model is able to upsample point clouds from all 7 categories with relatively high quality and accuracy. More visual results can be found in appendix XXX.

\subsection{Further discussions}\label{further}
According to the hypothesis we propose in section \ref{inner eval}, a mixture sampling method is designed to provide a potential better(superior) input point( cloud )distribution for upsampling. We introduce a new parameter, combining ratio $\alpha\in[0,1]$, to represent the percentage of points sampled(downsampled) from(by) curvature-based distribution.(strategy) The other points are downsampled(uniformly) from uniform distribution without repetition. As a parametric study, we create 11 groups of input point clouds(scatted?) from airplane category with $SF=8$ and an increment of $0.1$ in $\alpha$ each time. The test cases are identical to those we use in table \ref{tab: inner}.(?again) Figure XXX summarizes the relationship between $\alpha$ and the corresponding test chamfer loss. As shown, $\alpha=0.1$ or $\alpha=0.2$ both provide better(higher?) upsampling quality over the pure (?)uniform sampling method($\alpha=0$). The results exhibit the significance of points near the edges(?) on generalizing the whole shape of the point cloud.(?) Within a certain range of mixture(less than about $20\%$ in this case), the points sampled from curvature-based distribution(?) helps to decrease the Chamfer distance(?) in that the features around edges and corners are better represented.(?) But the input point is also becoming less uniform as $\alpha$ get larger. Eventually, the improvement resulted from edge points cannot make up for the increase in Chamfer ()loss caused by too few points on the flat surfaces. We can observe a gradual growth after a critical point($20\%$) in the curve shown in figure XXX.(感觉这理由是不是出现过)

As a comparison with the model we obtained from the best combining ratio, we utilize EAR\cite{XXX}, a state-of-the-art method for optimization-based point cloud upsampling method, to complete the same task. Figure XXX illustrates that our best model provides more precise upsampling results over EAR method. ()

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Conclusions}
This work presents a deep learning algorithm aiming at enriching the number of points in a sparse point cloud with flexible scaling factors. Through upsampling, our goal is to sense and supplement the point cloud with more information learned on other existing point clouds with similar global features. Instead of using any human defined priors, we take advantage of the outstanding ability of deep networks to obtain latent features for a certain object category. Then these latent features assist the point cloud upsampling
with correct category judgment so that some common global features learned from the same category can be naturally exploited.

We successively explore two different distributions for(of) the input point cloud sampling(s). Based on the results(outcomes), a further parametric study on the combining ratio for these two sampling methods is conducted to identify the benefit and side effect of curvature-based sampling. Within(with?) a certain combining rate, curvature-based sampling(distributed points) is capable of forming better(preciser?) description of the critical features around the edges(). Meanwhile, the descent of point density in areas far from edges causes(the scarcity of) less points in these areas during the upsampling, which unavoidably decrease the accuracy in current evaluation metric. However, in real application, the ultimate goal is usually to reconstruct a precise surface based on a dense point cloud. Less points in flat areas won't be a very severe problem since almost all the surfaces reconstruction methods assume smooth and flat surfaces between the given points. In this manner, our immediate next move is to find(define) more practical metrics to evaluate the resulting dense point cloud so that we can expand the applications of our algorithm.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Future Work}
Our current model is trained on point clouds sampled from PointNet. As we inspect the meshes utilized in our training, we find out that part of the meshes have flaws like open meshes or double-sided surface. These flaws lead to some incorrect normal calculation, which is a potential reason why normal information doesn't enhance the upsampling quality. An alternative way is to obtain the normal vectors only depending on the vertex coordinates. We believe it will bypass the defect in mesh surfaces and provide more precise normal vectors so that we can extensively verify its influence.  

Another limitation of our study is that our deep network is proficient at reconstruct the global features that are frequently occurred in the category. For those features that rarely exist or never occur in the training sets, the upsampling quality is not as good as the former ones. To address this problem, we can investigate the possibility of replenishing latent features learned from patch scale.

\begin{table*}[!htb]
\centering
\renewcommand{\arraystretch}{2}
\begin{tabular}{ |c||c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{3}{*}{} SF & \multicolumn{4}{c|}{2} & \multicolumn{4}{c|}{4} & \multicolumn{4}{c|}{8}\\ 
\cline{1-13}
                    Sample & \multicolumn{2}{c|}{Uniform} & \multicolumn{2}{c|}{CB} & \multicolumn{2}{c|}{Uniform} & \multicolumn{2}{c|}{CB} & \multicolumn{2}{c|}{Uniform} & \multicolumn{2}{c|}{CB}\\
\cline{1-13}
                    Normal & w/o & w/ & w/o & w/ & w/o & w/ & w/o & w/ & w/o & w/ & w/o & w/\\
\hline
Category & \multicolumn{12}{c|}{Accuracy($(\%)$)}\\
\hline
Airplane & 98.94 & 98.85 & 98.94 & 98.69 & 98.83 & 98.6 & 98.62 & 98.26 & 98.48 & 98.19 & 98.6 & 97.45\\
 \hline
Bench & 92.53 &	89.36 &	92.8 & 66.61 & 92.57 & 89.78 & 91.98 & 88.71 & 92.1 & 89.03 & 91.47 & 87.73\\ 
 \hline
Boat & 90.1 & 82.3 & 89.79 & 81.71 & 89.62 & 82.76 & 89.09 & 81.47 & 89.31 & 82.16 & 87.35 & 79.98\\ 
 \hline
Car & 91.94 & 91.45 & 91.91 & 91.77 & 91.83 & 91.24 & 91.18 & 90.45 & 91.39 & 90.56 & 90.53 & 89.64\\ 
 \hline
Chair & 80.17 &	79.11 &	80.02 &	79.63 &	79.7 &	78.96 &	74.56 &	73.6 & 78.98 & 78.33 & 72.91 & 70.94\\ 
 \hline
Lamp & 77.41 & 71.15 & 77.47 & 70.33 & 76.65 & 70.96 & 75.95 & 69.79 & 75.63 & 68.06 & 73.88 & 64.02\\ 
 \hline
Table & 87.15 &	86.81 &	86.87 &	86.58 &	86.79 &	86.35 &	85.13 &	84.63 &	86.22 &	85.87 &	83.79 &	83.3\\ 
 \hline
\end{tabular}
\caption{\label{tab: acc} Accuracy of networks trained on 7 categories respectively under twelve conditions.}
\end{table*}

\begin{table*}[!htb]
\centering
\renewcommand{\arraystretch}{2}
\begin{tabular}{ |c||c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{3}{*}{} SF & \multicolumn{4}{c|}{2} & \multicolumn{4}{c|}{4} & \multicolumn{4}{c|}{8}\\ 
\cline{1-13}
                    Sample & \multicolumn{2}{c|}{Uniform} & \multicolumn{2}{c|}{CB} & \multicolumn{2}{c|}{Uniform} & \multicolumn{2}{c|}{CB} & \multicolumn{2}{c|}{Uniform} & \multicolumn{2}{c|}{CB}\\
\cline{1-13}
                    Normal & w/o & w/ & w/o & w/ & w/o & w/ & w/o & w/ & w/o & w/ & w/o & w/\\
\hline
Category & \multicolumn{12}{c|}{Coverage($(\%)$)}\\
\hline
Airplane & 99.05 & 98.81 & 98.93 & 98.63 & 98.9 & 98.58 & 98.54 & 98.06 & 98.43 & 98 & 98.58 & 96.74\\
 \hline
Bench & 90.3 &	84.99 &	90.96 & 73.82 & 90.26 & 85.74 & 89.31 & 83.37 & 89.23 & 82.81 & 88.09 & 82.1\\ 
 \hline
Boat & 91.74 & 84.92 & 91.89 & 84.19 & 91.19 & 84.24 & 90.6 & 82.65 & 90.74 & 83.58 & 89.27 & 81.78\\ 
 \hline
Car & 94.64 & 93.83 & 94.38 & 94.16 & 94.43 & 93.53 & 93.46 & 92.68 & 93.94 & 92.71 & 92.59 & 91.42\\ 
 \hline
Chair & 81.26 &	79.71 &	80.51 &	80.05 & 80.48 &	80.18 &	76.76 &	75.52 & 79.25 & 78.5 & 75.02 & 73.48\\ 
 \hline
Lamp & 84.44 & 76.97 & 84.72 & 76.84 & 84.45 & 78.28 & 83.2 & 76.8 & 83.78 & 75.77 & 81.95 & 71.94\\ 
 \hline
Table & 81.4 &	81.15 &	81.39 &	81.04 &	81.09 &	80.72 &	79.16 &	78.41 &	80.64 &	79.97 &	77.17 &	77.07\\ 
 \hline
\end{tabular}
\caption{\label{tab: coverage} Coverage of networks trained on 7 categories respectively under twelve conditions.}
\end{table*}
